Development of deep biological ages aware of morbidity and mortality based on unsupervised and semi-supervised deep learning approaches

Background: While deep learning technology, which has the capability of obtaining latent representations based on large-scale data, can be a potential solution for the discovery of a novel aging biomarker, existing deep learning methods for biological age estimation usually depend on chronological ages and lack of consideration of mortality and morbidity that are the most significant outcomes of aging. Methods: This paper proposes a novel deep learning model to learn latent representations of biological aging in regard to subjects' morbidity and mortality. The model utilizes health check-up data in addition to morbidity and mortality information to learn the complex relationships between aging and measured clinical attributes. Findings: The proposed model is evaluated on a large dataset of general populations compared with KDM and other learning-based models. Results demonstrate that biological ages obtained by the proposed model have superior discriminability of subjects' morbidity and mortality.

==> 6_discussion.tex <==
% \begin{table}[t]
%     \centering
%     \setlength\tabcolsep{5pt}
%     \caption{CA prediction performance depending on overall morbidity of male subjects in root mean squared error (RMSE).}
%     \begin{tabular}{c c r r r r r r r r r}
%         \toprule \midrule
        
%         \multirow{2}{*}{Population} & \multirow{2}{*}{Model} & \multicolumn{3}{c}{\lfeature} & \multicolumn{3}{c}{\mfeature} & \multicolumn{3}{c}{\sfeature} \\ \cmidrule{3-11}
%         & & Healthy & Normal & Ill & Healthy & Normal & Ill &  Healthy & Normal & Ill \\ \midrule
        
%         \multirow{4}{*}{\textit{Whole}} & 
%             KDM & 43.02 & 39.39 & 44.80 & 21.26 & 24.37 & 26.77 & 17.62 & 22.27 & 23.75 \\
%             & CAC & 15.08 & 17.37 & 18.58 & 18.32 & 15.61 & 13.82 & 12.85 & 14.62 & 15.05 \\
%             & DNN & 7.31 & 7.50 & 7.75 & 9.88 & 9.95 & 9.55 & 10.48 & 9.97 & 9.74 \\ \cmidrule(lr){2-11}
%             & proposed & 5.19 & 5.55 & 6.17 & 7.18 & 7.42 & 7.50 & 8.20 & 7.92 & 7.98 \\ \midrule
            
%         \multirow{4}{*}{\textit{Average}} & 
%             KDM & 15.69 & 15.63 & 16.58 & 19.12 & 17.66 & 19.21 & 16.33 & 16.66 & 17.70 \\
%             & CAC & 15.02 & 14.79 & 13.64 & 17.92 & 15.26 & 12.60 & 14.99 & 15.55 & 15.14 \\
%             & DNN & 7.78 & 7.81 & 7.73 & 8.54 & 8.88 & 8.54 & 10.86 & 9.69 & 9.32 \\ \cmidrule(lr){2-11}
%             & proposed & 4.32 & 5.72 & 5.83 & 7.40 & 7.14 & 6.76 & 8.65 & 7.72 & 7.25 \\ \midrule
            
%         \multirow{4}{*}{\textit{Normal}} & 
%             KDM & 11.15 & 11.60 & \ood{12.59} & 13.96 & 14.27 & \ood{18.34} & 13.65 & 15.30 & \ood{17.60} \\
%             & CAC & 15.84 & 13.95 & \ood{12.77} & 15.30 & 13.55 & \ood{12.87} & 12.98 & 14.19 & \ood{14.10} \\
%             & DNN & 7.98 & 8.07 & \ood{8.65} & 8.57 & 9.19 & \ood{10.17} & 9.84 & 10.45 & \ood{10.60} \\ \cmidrule(lr){2-11}
%             & proposed & 13.53 & 14.46 & \ood{16.18} & 7.23 & 8.19 & \ood{8.81} & 8.27 & 8.45 & \ood{8.53} \\ \midrule
            
%         \multirow{4}{*}{\textit{Super normal}} & 
%             KDM & 9.71 & \ood{11.19} & \ood{12.54} & 13.09 & \ood{16.90} & \ood{22.71} & 14.25 & \ood{16.1} & \ood{18.76} \\
%             & CAC & 8.85 & \ood{9.98} & \ood{12.58} & 9.14 & \ood{9.52} & \ood{10.98} & 9.48 & \ood{9.54} & \ood{10.49} \\
%             & DNN & 8.97 & \ood{9.75} & \ood{12.54} & 9.59 & \ood{16.44} & \ood{25.61} & 11.93 & \ood{12.68} & \ood{15.08} \\ \cmidrule(lr){2-11}
%             & proposed & 9.10 & \ood{15.12} & \ood{16.98} & 9.26 & \ood{9.82} & \ood{12.2} & 9.59 & \ood{9.90} & \ood{11.01} \\ \midrule \bottomrule

%     \end{tabular}
%     \label{tab:ca_rmse}
% \end{table}

%Traditional methods for biological age estimation task include the multiple linear regression (MLR)\cite{hollingsworth1965correlations,dubina1983biological}, principal component analysis-based method (PCA) \cite{nakamura1988assessment,nakamura1989biological,  park2009developing,nakamura2007method,zhang2014select, nakamura2008sex} and Klemera and Doubal’s method (KDM) \cite{klemera2006anew}. They are all based on linear regression method but typically KDM is considered to be the most appropriate method for predicting mortality rate. 
\textbf{Evidence before this study}

 We searched PubMed for studies of machine learning-based biological age estimation with biomarkers
published from the inception of the database to Oct 22, 2022. We used the terms “deep learning” OR “machine learning” AND “Biological Age” AND "Biomarker". Our search yielded 31 results and the references of the identified studies were also reviewed. We also searched similarly for studies in the ML domain. We found multiple studies that developed ML models to estimate biological age using biomarker data but most of them employed traditional machine learning techniques which have relatively less computational power for modeling. There are a few studies that use relatively modern architectures but none of them considers morbidity and mortality conditions during training.
 %장점이 워낙 많아서 필요한 장점을 넣으면 될듯 modern ML technique, large dataset, CA를 예측하는게 아님
\\
\textbf{Somewhere in introduction/discussion}

Traditionally Klemera and Doubal's method (KDM) \cite{klemera2006anew} has been considered to be the most appropriate method for estimating biological age \cite{levine2013modeling,jia2017common, cho2010empirical}. Recently more advanced machine learning methods, in particular deep learning, have shown remarkable achievements in many areas including [relevant areas]. Similarly, biological age estimation via deep learning has been tried, for instance in \cite{bae2021comparison, putin2016deep,pyrkov2018extracting} with a certain amount of success. However, the models used in the previous studies are elementary by ML expert's standards. Our proposed model combines a Transformer, which has arguably been the most influential structure of machine learning for the past five years, and a Variational Autoencoder, also a frequently used architecture for generative modeling. Unlike previous approaches, not only do we use the up-to-date models used in the ML community nowadays, we directly guide the model to learn about the morbidity and mortality conditions by embedding clinical common sense in the training process. 

%(이 다음은 morbidity condtion/GAP 등등 모델 디자인 등이 아주 새롭다라는 내용등을 넣으면 자연스러울 것 같음) 


% 그래프 색 바꾸기 r package
% Kaplan-Meier curve variance 지우기 -> appendix로
% not dependent on CA, morbidity, mortality
% accessible and reasonable price
% generalizability -- different population
% weights for morbidity
% big cohort
% 전체, 당뇨 morbidity를 앞으로 빼기로
% 논문 제목에서 DBAge 빼기 -> lancet style 아님 -> new technology + big (and long) cohort + clinical implication + South Korea
% patient selection figure
% data distribution table (table 1)

